Decoupling Feature Extraction and Classification Layers for Calibrated Neural Networks

Deep Neural Networks (DNN) have shown great promise in many classification applications, yet are widely known to have poorly calibrated predictions when they are over-parametrized. Improving DNN calibration without comprising on model accuracy is of extreme importance and interest in safety critical applications such as in the health-care sector. In this work, we show that decoupling the training of feature extraction layers and classification layers in over-parametrized DNN architectures such as Wide Residual Networks (WRN) and Visual Transformers (ViT) significantly improves model calibration whilst retaining accuracy, and at a low training cost. In addition, we show that placing a Gaussian prior on the last hidden layer outputs of a DNN, and training the model variationally in the classification training stage, even further improves calibration. We illustrate these methods improve calibration across ViT and WRN architectures for several image classification benchmark datasets.

==> tables/BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{llll}
\toprule
 &  & OOD AUROC & OOD FPR95 \\
Dataset & Model &  &  \\
\midrule
\multirow[t]{5}{*}{CIFAR10} & V-TST, m=10 & 0.821$\pm$0.003 & 0.751$\pm$0.002 \\
 & V-TST, m=1 & 0.722$\pm$0.005 & 0.824$\pm$0.006 \\
 & TST & 0.874$\pm$0.002 & 0.699$\pm$0.009 \\
 & Temp. WRN & 0.872 & 0.746 \\
 & WRN & 0.891 & 0.653 \\
\midrule
\multirow[t]{5}{*}{CIFAR100} & V-TST, m=10 & 0.791$\pm$0.002 & 0.809$\pm$0.004 \\
 & V-TST, m=1 & 0.783$\pm$0.004 & 0.822$\pm$0.006 \\
 & TST & 0.823$\pm$0.002 & 0.764$\pm$0.006 \\
 & Temp. WRN & 0.778 & 0.816 \\
 & WRN & 0.785 & 0.892 \\
\midrule
\multirow[t]{5}{*}{SVHN} & V-TST, m=10 & 0.872$\pm$0.004 & 0.537$\pm$0.003 \\
 & V-TST, m=1 & 0.859$\pm$0.004 & 0.549$\pm$0.006 \\
 & TST & 0.935$\pm$0.001 & 0.415$\pm$0.006 \\
 & Temp. WRN & 0.934 & 0.461 \\
 & WRN & 0.945 & 0.344 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_BEST_BNN_IN_metrics.tex <==
\begin{tabular}{lcccccc}
\toprule
 & Accuracy & ECE & MCE & Brier & Train NLL & Test NLL \\
Model &  &  &  &  &  &  \\
\midrule
TST Z128 & \bfseries 92.586$\pm$0.0208 & 2.18$\pm$0.353 & 14.89$\pm$2.249 & \bfseries 0.011$\pm$6e-05 & \bfseries 0.057$\pm$0.00023 & \bfseries 0.248$\pm$0.004 \\
V-TST Z32 & 91.095$\pm$0.0604 & \bfseries 1.520$\pm$0.144 & \bfseries 14.770$\pm$1.781 & 0.0142$\pm$8e-05 & 0.1125$\pm$0.00099 & 0.3732$\pm$0.00426 \\
WRN 28-10 & 92.53$\pm$nan & 5.88$\pm$nan & 35.84$\pm$nan & 0.013$\pm$nan & 0.1038$\pm$nan & 0.4944$\pm$nan \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
 & OOD AUROC & OOD FPR95 \\
Model &  &  \\
\midrule
TST Z128 & 0.874$\pm$0.0022 & 0.699$\pm$0.009 \\
V-TST Z32 & 0.722$\pm$0.0053 & 0.824$\pm$0.0065 \\
WRN 28-10 & \bfseries 0.891$\pm$nan & \bfseries 0.653$\pm$nan \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_BEST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
 & SHIFT ECE & SHIFT MCE \\
Model &  &  \\
\midrule
TST Z128 & \bfseries 11.620$\pm$0.752 & 25.39$\pm$1.74 \\
V-TST Z32 & 12.89$\pm$0.297 & \bfseries 21.010$\pm$0.58 \\
WRN 28-10 & 20.27$\pm$nan & 45.06$\pm$nan \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_BNN_metrics.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         Accuracy &              ECE &               MCE &            Brier &              NLL \\
Model                                  &                  &                  &                   &                  &                  \\
\midrule
CondVAE-wang2023-DropRate00-Z128-seed1 &          0.95380 &          3.16112 &          73.50188 &          0.00789 &          0.22663 \\
CondVAE-wang2023-DropRate00-Z2-seed1   &          0.81780 &          5.54212 &          15.15805 &          0.02792 &          0.72067 \\
CondVAE-wang2023-DropRate00-Z32-seed1  &  \bfseries 0.955 &          2.83231 &          82.97464 &          0.00759 &          0.21634 \\
CondVAE-wang2023-DropRate02-Z128-seed1 &  \bfseries 0.955 &          3.03962 &          30.46379 &          0.00775 &          0.22053 \\
CondVAE-wang2023-DropRate02-Z2-seed1   &          0.81650 &          4.78844 &  \bfseries 11.889 &          0.02819 &          0.71662 \\
CondVAE-wang2023-DropRate02-Z32-seed1  &          0.95400 &          2.94535 &          31.37523 &          0.00766 &          0.21652 \\
CondVAE-wang2023-DropRate05-Z128-seed1 &  \bfseries 0.955 &  \bfseries 2.354 &          18.46937 &  \bfseries 0.007 &  \bfseries 0.191 \\
CondVAE-wang2023-DropRate05-Z2-seed1   &          0.81410 &         10.33272 &          31.84117 &          0.02936 &          0.85866 \\
CondVAE-wang2023-DropRate05-Z32-seed1  &          0.95400 &          3.00787 &          26.38475 &          0.00768 &          0.22205 \\
CondVAE-wang2023-DropRate08-Z128-seed1 &  \bfseries 0.955 &          3.27215 &          28.67978 &          0.00789 &          0.24902 \\
CondVAE-wang2023-DropRate08-Z2-seed1   &          0.79490 &          5.83840 &          17.13515 &          0.03145 &          0.80606 \\
CondVAE-wang2023-DropRate08-Z32-seed1  &          0.95440 &          3.14009 &          32.60792 &          0.00774 &          0.23025 \\
Wang2023                               &          0.95160 &         18.40900 &          33.08432 &          0.01222 &          0.33405 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_CNN_BNN_IN_metrics.tex <==
\begin{tabular}{lcccccc}
\toprule
 & Accuracy & ECE & MCE & Brier & Train NLL & Test NLL \\
Model &  &  &  &  &  &  \\
\midrule
CNN & 72.48$\pm$nan & 1.04$\pm$nan & 19.89$\pm$nan & 0.0386$\pm$nan & 0.7132$\pm$nan & 0.81$\pm$nan \\
TST Z128 & 73.97$\pm$0.196 & 2.92$\pm$0.332 & 18.66$\pm$0.39 & 0.0361$\pm$0.00014 & 0.5951$\pm$0.00277 & 0.7593$\pm$0.00269 \\
TST Z256 & 74.86$\pm$0.111 & 3.9$\pm$0.085 & 15.29$\pm$3.719 & \bfseries 0.035$\pm$5e-05 & 0.5326$\pm$0.00629 & 0.7478$\pm$0.00071 \\
TST Z32 & 70.77$\pm$0.177 & \bfseries 0.760$\pm$0.172 & 7.79$\pm$4.67 & 0.0399$\pm$9e-05 & 0.7706$\pm$0.00245 & 0.834$\pm$0.00197 \\
TST Z512 & 74.84$\pm$0.156 & 2.58$\pm$0.413 & 22.87$\pm$4.241 & \bfseries 0.035$\pm$7e-05 & 0.5596$\pm$0.01376 & \bfseries 0.740$\pm$0.00175 \\
TST Z8 & 65.51$\pm$0.151 & 2.39$\pm$0.194 & 14.45$\pm$5.075 & 0.0467$\pm$0.00019 & 0.9707$\pm$0.00439 & 0.9889$\pm$0.00548 \\
V-TST Z128, m=1 & 73.22$\pm$0.122 & 1.61$\pm$0.299 & 9.08$\pm$5.473 & 0.0371$\pm$9e-05 & 0.6416$\pm$0.00202 & 0.7847$\pm$0.00216 \\
V-TST Z256, m=1 & 74.23$\pm$0.136 & 3.65$\pm$0.278 & 22.5$\pm$4.379 & 0.0356$\pm$0.00012 & 0.5368$\pm$0.00294 & 0.7563$\pm$0.00417 \\
V-TST Z32, m=1 & 66.74$\pm$0.282 & 1.09$\pm$0.209 & 7.81$\pm$2.272 & 0.0447$\pm$0.00019 & 0.8981$\pm$0.0069 & 0.953$\pm$0.00243 \\
V-TST Z512, m=1 & \bfseries 74.870$\pm$0.152 & 5.77$\pm$0.248 & 21.0$\pm$5.511 & 0.0357$\pm$0.00021 & \bfseries 0.444$\pm$0.00305 & 0.7735$\pm$0.00357 \\
V-TST Z8, m=1 & 53.54$\pm$0.532 & 3.13$\pm$0.393 & \bfseries 6.620$\pm$0.857 & 0.0595$\pm$0.00033 & 1.2905$\pm$0.00873 & 1.3107$\pm$0.00579 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_CNN_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
 & OOD AUROC & OOD FPR95 \\
Model &  &  \\
\midrule
CNN & \bfseries 0.738$\pm$nan & \bfseries 0.885$\pm$nan \\
TST Z128 & 0.727$\pm$0.0042 & 0.901$\pm$0.001 \\
TST Z256 & 0.721$\pm$0.0054 & 0.898$\pm$0.0068 \\
TST Z32 & 0.73$\pm$0.0031 & 0.911$\pm$0.0055 \\
TST Z512 & 0.721$\pm$0.0017 & 0.905$\pm$0.0006 \\
TST Z8 & 0.699$\pm$0.0092 & 0.934$\pm$0.0077 \\
V-TST Z128, m=1 & 0.689$\pm$0.012 & 0.936$\pm$0.0099 \\
V-TST Z256, m=1 & 0.685$\pm$0.0115 & 0.936$\pm$0.0082 \\
V-TST Z32, m=1 & 0.645$\pm$0.0054 & 0.946$\pm$0.0047 \\
V-TST Z512, m=1 & 0.688$\pm$0.0028 & 0.93$\pm$0.0023 \\
V-TST Z8, m=1 & 0.609$\pm$0.0148 & 0.944$\pm$0.0058 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_CNN_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
 & SHIFT ECE & SHIFT MCE \\
Model &  &  \\
\midrule
CNN & 9.13$\pm$nan & 11.8$\pm$nan \\
TST Z128 & 9.85$\pm$0.182 & 13.68$\pm$0.296 \\
TST Z256 & 11.03$\pm$0.257 & 15.46$\pm$0.225 \\
TST Z32 & 7.02$\pm$0.084 & 9.39$\pm$0.349 \\
TST Z512 & 9.54$\pm$0.611 & 13.37$\pm$0.827 \\
TST Z8 & 5.53$\pm$0.24 & 8.47$\pm$0.071 \\
V-TST Z128, m=1 & 8.18$\pm$0.129 & 11.15$\pm$0.079 \\
V-TST Z256, m=1 & 10.23$\pm$0.336 & 14.68$\pm$0.535 \\
V-TST Z32, m=1 & 6.33$\pm$0.232 & 9.0$\pm$0.315 \\
V-TST Z512, m=1 & 13.31$\pm$0.142 & 19.75$\pm$0.251 \\
V-TST Z8, m=1 & \bfseries 4.230$\pm$0.038 & \bfseries 5.900$\pm$0.197 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_WRN_BNN_IN_metrics.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         Accuracy &              ECE &               MCE &            Brier &              NLL \\
Model                                  &                  &                  &                   &                  &                  \\
\midrule
CondVAE-WRN-DropRate00-Z128-seed1      &  \bfseries 0.909 &  \bfseries 3.793 &          16.44534 &  \bfseries 0.017 &  \bfseries 0.510 \\
CondVAE-WRN-DropRate00-Z128-seed1-LAST &          0.90810 &          9.01990 &          56.71228 &          0.01809 &          1.51839 \\
CondVAE-WRN-DropRate00-Z2-seed1        &          0.90270 &         35.35309 &          55.11271 &          0.03691 &          0.90593 \\
CondVAE-WRN-DropRate00-Z2-seed1-LAST   &          0.90300 &          7.72196 &          44.19723 &          0.01805 &          1.13682 \\
CondVAE-WRN-DropRate00-Z32-seed1       &  \bfseries 0.909 &          6.29863 &  \bfseries 13.602 &  \bfseries 0.017 &          0.56721 \\
CondVAE-WRN-DropRate00-Z32-seed1-LAST  &  \bfseries 0.909 &          8.91054 &          49.51017 &          0.01795 &          1.40931 \\
CondVAE-WRN-DropRate02-Z128-seed1      &  \bfseries 0.909 &          4.13841 &          38.22795 &  \bfseries 0.017 &          0.51367 \\
CondVAE-WRN-DropRate02-Z128-seed1-LAST &          0.90830 &          9.04737 &          39.46790 &          0.01818 &          1.54449 \\
CondVAE-WRN-DropRate02-Z2-seed1        &          0.90180 &         24.38788 &          42.98495 &          0.02892 &          0.83997 \\
CondVAE-WRN-DropRate02-Z2-seed1-LAST   &          0.90330 &          7.64644 &          52.34021 &          0.01799 &          1.12984 \\
CondVAE-WRN-DropRate02-Z32-seed1       &  \bfseries 0.909 &          6.47955 &          25.83405 &  \bfseries 0.017 &          0.56327 \\
CondVAE-WRN-DropRate02-Z32-seed1-LAST  &  \bfseries 0.909 &          8.91651 &          39.59374 &          0.01794 &          1.40440 \\
CondVAE-WRN-DropRate05-Z128-seed1      &          0.90790 &          4.34407 &          39.13937 &  \bfseries 0.017 &          0.52154 \\
CondVAE-WRN-DropRate05-Z128-seed1-LAST &          0.90790 &          9.04741 &          49.31107 &          0.01821 &          1.54648 \\
CondVAE-WRN-DropRate05-Z2-seed1        &          0.90290 &         19.00352 &          40.85639 &          0.02532 &          0.79226 \\
CondVAE-WRN-DropRate05-Z2-seed1-LAST   &          0.90360 &          7.58992 &          42.86601 &          0.01793 &          1.10494 \\
CondVAE-WRN-DropRate05-Z32-seed1       &          0.90820 &          6.43699 &          27.04051 &  \bfseries 0.017 &          0.57166 \\
CondVAE-WRN-DropRate05-Z32-seed1-LAST  &  \bfseries 0.909 &          8.88069 &          37.31249 &          0.01791 &          1.41231 \\
CondVAE-WRN-DropRate08-Z128-seed1      &          0.90740 &          4.44652 &          22.37766 &  \bfseries 0.017 &          0.51933 \\
CondVAE-WRN-DropRate08-Z128-seed1-LAST &          0.90800 &          9.04560 &          57.14469 &          0.01819 &          1.58780 \\
CondVAE-WRN-DropRate08-Z2-seed1        &          0.90170 &         20.54395 &          37.77272 &          0.02660 &          0.81285 \\
CondVAE-WRN-DropRate08-Z2-seed1-LAST   &          0.90320 &          7.70339 &          62.31697 &          0.01803 &          1.12991 \\
CondVAE-WRN-DropRate08-Z32-seed1       &          0.90770 &          6.48232 &          28.11965 &  \bfseries 0.017 &          0.57103 \\
CondVAE-WRN-DropRate08-Z32-seed1-LAST  &          0.90730 &          9.05835 &          51.55667 &          0.01824 &          1.42614 \\
WRN-Base                               &          0.90460 &          7.39412 &          37.91238 &  \bfseries 0.017 &          0.57115 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_WRN_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &        OOD AUROC &        OOD FPR95 \\
Model                                  &                  &                  \\
\midrule
CondVAE-WRN-DropRate00-Z128-seed1      &          0.79384 &          0.83895 \\
CondVAE-WRN-DropRate00-Z128-seed1-LAST &          0.83301 &          0.78075 \\
CondVAE-WRN-DropRate00-Z2-seed1        &          0.77071 &          0.74961 \\
CondVAE-WRN-DropRate00-Z2-seed1-LAST   &          0.73871 &          0.71681 \\
CondVAE-WRN-DropRate00-Z32-seed1       &          0.82332 &          0.81719 \\
CondVAE-WRN-DropRate00-Z32-seed1-LAST  &          0.84710 &          0.77020 \\
CondVAE-WRN-DropRate02-Z128-seed1      &          0.79712 &          0.83318 \\
CondVAE-WRN-DropRate02-Z128-seed1-LAST &          0.78862 &          0.80578 \\
CondVAE-WRN-DropRate02-Z2-seed1        &          0.74175 &          0.75061 \\
CondVAE-WRN-DropRate02-Z2-seed1-LAST   &          0.72589 &  \bfseries 0.701 \\
CondVAE-WRN-DropRate02-Z32-seed1       &          0.83828 &          0.80670 \\
CondVAE-WRN-DropRate02-Z32-seed1-LAST  &          0.84778 &          0.76887 \\
CondVAE-WRN-DropRate05-Z128-seed1      &          0.78681 &          0.84039 \\
CondVAE-WRN-DropRate05-Z128-seed1-LAST &          0.81209 &          0.79973 \\
CondVAE-WRN-DropRate05-Z2-seed1        &          0.78135 &          0.72980 \\
CondVAE-WRN-DropRate05-Z2-seed1-LAST   &          0.73810 &          0.70568 \\
CondVAE-WRN-DropRate05-Z32-seed1       &          0.82404 &          0.81441 \\
CondVAE-WRN-DropRate05-Z32-seed1-LAST  &          0.83677 &          0.76238 \\
CondVAE-WRN-DropRate08-Z128-seed1      &          0.77539 &          0.84858 \\
CondVAE-WRN-DropRate08-Z128-seed1-LAST &          0.78099 &          0.82463 \\
CondVAE-WRN-DropRate08-Z2-seed1        &          0.76975 &          0.73049 \\
CondVAE-WRN-DropRate08-Z2-seed1-LAST   &          0.73956 &          0.71803 \\
CondVAE-WRN-DropRate08-Z32-seed1       &          0.83451 &          0.81011 \\
CondVAE-WRN-DropRate08-Z32-seed1-LAST  &  \bfseries 0.866 &  \bfseries 0.701 \\
WRN_Base                               &          0.86175 &          0.71450 \\
\bottomrule
\end{tabular}


==> tables/CIFAR10_WRN_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &        SHIFT ECE &         SHIFT MCE \\
Model                                  &                  &                   \\
\midrule
CondVAE-WRN-DropRate00-Z128-seed1      &         16.67596 &          28.91946 \\
CondVAE-WRN-DropRate00-Z128-seed1-LAST &         24.39021 &          51.32581 \\
CondVAE-WRN-DropRate00-Z2-seed1        &         22.67845 &          39.29760 \\
CondVAE-WRN-DropRate00-Z2-seed1-LAST   &         22.65636 &          55.83237 \\
CondVAE-WRN-DropRate00-Z32-seed1       &         20.27039 &          38.19189 \\
CondVAE-WRN-DropRate00-Z32-seed1-LAST  &         24.24135 &          52.73468 \\
CondVAE-WRN-DropRate02-Z128-seed1      &         17.71589 &          30.32231 \\
CondVAE-WRN-DropRate02-Z128-seed1-LAST &         24.57889 &          52.43281 \\
CondVAE-WRN-DropRate02-Z2-seed1        &         12.53008 &          27.02288 \\
CondVAE-WRN-DropRate02-Z2-seed1-LAST   &         22.68418 &          56.06058 \\
CondVAE-WRN-DropRate02-Z32-seed1       &         20.56124 &          38.17421 \\
CondVAE-WRN-DropRate02-Z32-seed1-LAST  &         24.36524 &          51.65735 \\
CondVAE-WRN-DropRate05-Z128-seed1      &         18.07170 &          30.05764 \\
CondVAE-WRN-DropRate05-Z128-seed1-LAST &         24.71034 &          54.81312 \\
CondVAE-WRN-DropRate05-Z2-seed1        &  \bfseries 7.141 &          25.64265 \\
CondVAE-WRN-DropRate05-Z2-seed1-LAST   &         22.70883 &          55.94867 \\
CondVAE-WRN-DropRate05-Z32-seed1       &         20.59760 &          39.21906 \\
CondVAE-WRN-DropRate05-Z32-seed1-LAST  &         24.33166 &          70.96033 \\
CondVAE-WRN-DropRate08-Z128-seed1      &         18.02666 &          29.88127 \\
CondVAE-WRN-DropRate08-Z128-seed1-LAST &         24.69452 &          52.08811 \\
CondVAE-WRN-DropRate08-Z2-seed1        &          8.06386 &  \bfseries 17.880 \\
CondVAE-WRN-DropRate08-Z2-seed1-LAST   &         22.80390 &          55.67095 \\
CondVAE-WRN-DropRate08-Z32-seed1       &         20.86271 &          38.72018 \\
CondVAE-WRN-DropRate08-Z32-seed1-LAST  &         24.53684 &          51.96549 \\
WRN_Base                               &         19.52035 &          43.52953 \\
\bottomrule
\end{tabular}


==> tables/CNN_ABLATION_BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{llll}
\toprule
 & OOD AUROC & OOD FPR95 \\
Model &  &  \\
\midrule
V-TST, m=10 & 0.713$\pm$0.002 & 0.9$\pm$0.002 \\
V-TST, m=1 & 0.689$\pm$0.012 & 0.936$\pm$0.01 \\
TST & 0.73$\pm$0.003 & 0.911$\pm$0.006 \\
CNN & 0.704$\pm$0.034 & 0.917$\pm$0.032 \\
\bottomrule
\end{tabular}


==> tables/CNN_ABLATION_BEST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{llll}
\toprule
 & SHIFT ECE & SHIFT MCE \\
Model &  &  \\
\midrule
V-TST, m=10 & 10.06$\pm$0.16 & 14.56$\pm$0.27 \\
V-TST, m=1 & 8.18$\pm$0.13 & 11.15$\pm$0.08 \\
TST & 7.02$\pm$0.08 & 9.39$\pm$0.35 \\
CNN & 9.13$\pm$0.0 & 11.8$\pm$0.0 \\
\bottomrule
\end{tabular}


==> tables/ETE_ABLATION_BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{llll}
\toprule
 & OOD AUROC & OOD FPR95 \\
Model &  &  \\
\midrule
Var. E2E, m=10 & 0.694 & 0.756 \\
Var. E2E, m=1 & 0.713 & 0.809 \\
E2E & 0.922 & 0.494 \\
\bottomrule
\end{tabular}


==> tables/ETE_ABLATION_BEST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{llll}
\toprule
 & SHIFT ECE & SHIFT MCE \\
Model &  &  \\
\midrule
Var. E2E, m=10 & 19.83 & 37.32 \\
Var. E2E, m=1 & 21.63 & 34.72 \\
E2E & 20.67 & 47.13 \\
\bottomrule
\end{tabular}


==> tables/ETE_intro_ABLATION_BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{llcc}
\toprule
 & OOD AUROC & OOD FPR95 \\
Model &  &  \\
\midrule
TST & 0.887$\pm$0.001 & 0.678$\pm$0.006 \\
E2E & 0.873$\pm$nan & 0.733$\pm$nan \\
\bottomrule
\end{tabular}


==> tables/ETE_intro_ABLATION_BEST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{llcc}
\toprule
 & SHIFT ECE & SHIFT MCE \\
Model &  &  \\
\midrule
TST & 12.51$\pm$0.47 & 26.35$\pm$1.15 \\
E2E & 20.67$\pm$nan & 47.13$\pm$nan \\
\bottomrule
\end{tabular}


==> tables/ETE_intro_ABLATION_BNN_IN_metrics.tex <==
\begin{tabular}{llccc}
\toprule
 & Accuracy & ECE & MCE \\
Model &  &  &  \\
\midrule
TST & 91.61$\pm$0.03 & 2.87$\pm$0.2 & 15.54$\pm$1.91 \\
E2E & 91.41$\pm$nan & 6.74$\pm$nan & 37.22$\pm$nan \\
\bottomrule
\end{tabular}


==> tables/FMNIST_BNN_IN_metrics.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         Accuracy &              ECE &               MCE &            Brier &              NLL \\
Model                         &                  &                  &                   &                  &                  \\
\midrule
CondVAE-DropRate00-Z128-seed1 &          0.89700 &          4.98461 &          26.13207 &          0.01686 &          0.43642 \\
CondVAE-DropRate00-Z2-seed1   &          0.86360 &         35.10547 &          47.57087 &          0.04001 &          0.96982 \\
CondVAE-DropRate00-Z32-seed1  &  \bfseries 0.898 &          3.01573 &          21.52915 &  \bfseries 0.016 &          0.40506 \\
CondVAE-DropRate02-Z128-seed1 &  \bfseries 0.898 &          4.88103 &          25.39970 &          0.01682 &          0.43674 \\
CondVAE-DropRate02-Z2-seed1   &          0.85720 &         34.95720 &          46.83702 &          0.04053 &          0.98508 \\
CondVAE-DropRate02-Z32-seed1  &          0.89740 &          5.89991 &          30.83282 &          0.01705 &          0.44087 \\
CondVAE-DropRate05-Z128-seed1 &          0.89740 &          4.82422 &          80.99610 &          0.01684 &          0.43952 \\
CondVAE-DropRate05-Z2-seed1   &          0.85180 &         30.99807 &          46.05749 &          0.03848 &          0.96570 \\
CondVAE-DropRate05-Z32-seed1  &          0.89720 &          3.24253 &          21.49452 &  \bfseries 0.016 &          0.41001 \\
CondVAE-DropRate08-Z128-seed1 &          0.89750 &          4.96608 &          80.30004 &          0.01687 &          0.44702 \\
CondVAE-DropRate08-Z2-seed1   &          0.85810 &         28.58072 &          46.75071 &          0.03633 &          0.93837 \\
CondVAE-DropRate08-Z32-seed1  &          0.89710 &          3.32392 &          22.86654 &  \bfseries 0.016 &          0.41346 \\
WRN-Base                      &          0.88380 &  \bfseries 1.147 &  \bfseries 18.876 &          0.01712 &  \bfseries 0.348 \\
\bottomrule
\end{tabular}


==> tables/FMNIST_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &        OOD AUROC &        OOD FPR95 \\
Model                         &                  &                  \\
\midrule
CondVAE-DropRate00-Z128-seed1 &          0.91512 &          0.53690 \\
CondVAE-DropRate00-Z2-seed1   &          0.73418 &          0.83695 \\
CondVAE-DropRate00-Z32-seed1  &          0.93275 &          0.48215 \\
CondVAE-DropRate02-Z128-seed1 &          0.91383 &          0.54625 \\
CondVAE-DropRate02-Z2-seed1   &          0.75365 &          0.74850 \\
CondVAE-DropRate02-Z32-seed1  &          0.92975 &          0.50855 \\
CondVAE-DropRate05-Z128-seed1 &          0.92117 &          0.52705 \\
CondVAE-DropRate05-Z2-seed1   &          0.78604 &          0.61245 \\
CondVAE-DropRate05-Z32-seed1  &          0.93234 &          0.48400 \\
CondVAE-DropRate08-Z128-seed1 &          0.91826 &          0.54360 \\
CondVAE-DropRate08-Z2-seed1   &          0.74962 &          0.75205 \\
CondVAE-DropRate08-Z32-seed1  &          0.93304 &          0.48755 \\
WRN-Base                      &  \bfseries 0.969 &  \bfseries 0.181 \\
\bottomrule
\end{tabular}


==> tables/FMNIST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &        SHIFT ECE &         SHIFT MCE \\
Model                         &                  &                   \\
\midrule
CondVAE-DropRate00-Z128-seed1 &         37.12386 &          49.77684 \\
CondVAE-DropRate00-Z2-seed1   &         10.91934 &          18.59212 \\
CondVAE-DropRate00-Z32-seed1  &         33.10500 &          50.13700 \\
CondVAE-DropRate02-Z128-seed1 &         37.36599 &          48.74593 \\
CondVAE-DropRate02-Z2-seed1   &  \bfseries 9.964 &          21.62889 \\
CondVAE-DropRate02-Z32-seed1  &         39.19614 &          50.65845 \\
CondVAE-DropRate05-Z128-seed1 &         36.79557 &          49.69537 \\
CondVAE-DropRate05-Z2-seed1   &         13.46143 &  \bfseries 16.462 \\
CondVAE-DropRate05-Z32-seed1  &         32.60740 &          51.70703 \\
CondVAE-DropRate08-Z128-seed1 &         36.58685 &          49.29942 \\
CondVAE-DropRate08-Z2-seed1   &         13.77910 &          71.55941 \\
CondVAE-DropRate08-Z32-seed1  &         33.10500 &          50.49510 \\
WRN-Base                      &         33.86308 &          49.86988 \\
\bottomrule
\end{tabular}


==> tables/FMNIST_autoattack_results.tex <==
\begin{tabular}{lcccc}
\toprule
{} &   Clean Accuracy & $\epsilon=\frac{4}{255}$ & $\epsilon=\frac{8}{255}$ &   $\epsilon=0.3$ \\
Model                          &                  &                          &                          &                  \\
\midrule
CNN                            &  \bfseries 0.908 &                    0.655 &                    0.384 &            0.000 \\
AdvCNN                         &            0.901 &                    0.492 &                    0.292 &            0.053 \\
CondVAE-NoDrop-Z32             &            0.906 &                    0.690 &                    0.439 &            0.000 \\
CondVAE-AdvQYX-NoDrop-Z32      &            0.901 &                    0.500 &                    0.355 &            0.135 \\
CondVAE-NoDrop-Z128            &            0.906 &          \bfseries 0.691 &          \bfseries 0.442 &            0.000 \\
CondVAE-AdvQYX-NoDrop-Z128     &            0.901 &                    0.503 &                    0.357 &  \bfseries 0.140 \\
CondVAE-DropRate02-Z32         &            0.906 &                    0.690 &                    0.440 &            0.000 \\
CondVAE-AdvQYX-DropRate02-Z32  &            0.900 &                    0.499 &                    0.361 &            0.135 \\
CondVAE-DropRate02-Z128        &            0.906 &          \bfseries 0.691 &                    0.441 &            0.000 \\
CondVAE-AdvQYX-DropRate02-Z128 &            0.901 &                    0.502 &                    0.360 &            0.136 \\
CondVAE-DropRate05-Z32         &            0.906 &                    0.690 &                    0.440 &            0.000 \\
CondVAE-AdvQYX-DropRate05-Z32  &            0.901 &                    0.501 &                    0.355 &            0.131 \\
CondVAE-DropRate05-Z128        &            0.905 &                    0.690 &                    0.439 &            0.000 \\
CondVAE-AdvQYX-DropRate05-Z128 &            0.901 &                    0.499 &                    0.350 &            0.124 \\
CondVAE-DropRate08-Z32         &            0.906 &                    0.689 &                    0.438 &            0.000 \\
CondVAE-AdvQYX-DropRate08-Z32  &            0.900 &                    0.497 &                    0.349 &            0.128 \\
CondVAE-DropRate08-Z128        &            0.905 &                    0.688 &                    0.438 &            0.000 \\
CondVAE-AdvQYX-DropRate08-Z128 &            0.900 &                    0.497 &                    0.349 &            0.130 \\
\bottomrule
\end{tabular}


==> tables/MNIST_BNN_IN_metrics.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         Accuracy &              ECE &               MCE &            Brier &              NLL \\
Model                         &                  &                  &                   &                  &                  \\
\midrule
CondVAE-DropRate00-Z128-seed1 &  \bfseries 0.994 &          0.52164 &          74.86594 &  \bfseries 0.001 &          0.04398 \\
CondVAE-DropRate00-Z2-seed1   &          0.99150 &         13.93574 &          41.95844 &          0.00825 &          0.21860 \\
CondVAE-DropRate00-Z32-seed1  &  \bfseries 0.994 &          0.54554 &          40.54808 &  \bfseries 0.001 &          0.05461 \\
CondVAE-DropRate02-Z128-seed1 &  \bfseries 0.994 &          0.53747 &          65.94275 &  \bfseries 0.001 &          0.04366 \\
CondVAE-DropRate02-Z2-seed1   &          0.99160 &          8.46881 &          25.51012 &          0.00395 &          0.14970 \\
CondVAE-DropRate02-Z32-seed1  &          0.99350 &          0.61071 &          70.05146 &  \bfseries 0.001 &          0.05739 \\
CondVAE-DropRate05-Z128-seed1 &  \bfseries 0.994 &          0.52384 &          52.08219 &  \bfseries 0.001 &          0.04568 \\
CondVAE-DropRate05-Z2-seed1   &          0.99140 &          5.54967 &          39.99439 &          0.00256 &          0.12622 \\
CondVAE-DropRate05-Z32-seed1  &          0.99350 &          0.59683 &          50.73436 &  \bfseries 0.001 &          0.05707 \\
CondVAE-DropRate08-Z128-seed1 &  \bfseries 0.994 &          0.47092 &          30.82274 &  \bfseries 0.001 &          0.04106 \\
CondVAE-DropRate08-Z2-seed1   &          0.99190 &          6.57827 &          38.57295 &          0.00328 &          0.13076 \\
CondVAE-DropRate08-Z32-seed1  &  \bfseries 0.994 &          0.58985 &          54.16973 &  \bfseries 0.001 &          0.05678 \\
WRN-Base                      &  \bfseries 0.994 &  \bfseries 0.223 &  \bfseries 23.963 &  \bfseries 0.001 &  \bfseries 0.020 \\
\bottomrule
\end{tabular}


==> tables/MNIST_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &        OOD AUROC &        OOD FPR95 \\
Model                         &                  &                  \\
\midrule
CondVAE-DropRate00-Z128-seed1 &          0.88711 &          0.30555 \\
CondVAE-DropRate00-Z2-seed1   &          0.74684 &          0.77650 \\
CondVAE-DropRate00-Z32-seed1  &          0.85241 &          0.31470 \\
CondVAE-DropRate02-Z128-seed1 &          0.90158 &          0.25835 \\
CondVAE-DropRate02-Z2-seed1   &          0.78974 &          0.72470 \\
CondVAE-DropRate02-Z32-seed1  &          0.85854 &          0.29475 \\
CondVAE-DropRate05-Z128-seed1 &          0.87466 &          0.31710 \\
CondVAE-DropRate05-Z2-seed1   &          0.83491 &          0.68770 \\
CondVAE-DropRate05-Z32-seed1  &          0.89229 &          0.27515 \\
CondVAE-DropRate08-Z128-seed1 &          0.87036 &          0.32320 \\
CondVAE-DropRate08-Z2-seed1   &          0.80901 &          0.68690 \\
CondVAE-DropRate08-Z32-seed1  &          0.89967 &          0.25110 \\
WRN-Base                      &  \bfseries 0.930 &  \bfseries 0.180 \\
\bottomrule
\end{tabular}


==> tables/MNIST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &         SHIFT ECE &         SHIFT MCE \\
Model                         &                   &                   \\
\midrule
CondVAE-DropRate00-Z128-seed1 &          46.13864 &          68.20023 \\
CondVAE-DropRate00-Z2-seed1   &  \bfseries 30.137 &          52.48224 \\
CondVAE-DropRate00-Z32-seed1  &          47.48224 &          69.61353 \\
CondVAE-DropRate02-Z128-seed1 &          46.00935 &          66.56991 \\
CondVAE-DropRate02-Z2-seed1   &          34.73636 &  \bfseries 46.891 \\
CondVAE-DropRate02-Z32-seed1  &          47.42991 &          66.69210 \\
CondVAE-DropRate05-Z128-seed1 &          46.51664 &          65.94723 \\
CondVAE-DropRate05-Z2-seed1   &          38.01282 &          70.06565 \\
CondVAE-DropRate05-Z32-seed1  &          47.41833 &          67.78459 \\
CondVAE-DropRate08-Z128-seed1 &          45.53412 &          67.50729 \\
CondVAE-DropRate08-Z2-seed1   &          37.28195 &          58.44398 \\
CondVAE-DropRate08-Z32-seed1  &          47.39749 &          67.54560 \\
WRN-Base                      &          36.55066 &          58.13984 \\
\bottomrule
\end{tabular}


==> tables/MNIST_autoattack_results.tex <==
\begin{tabular}{lcccc}
\toprule
{} &   Clean Accuracy & $\epsilon=\frac{4}{255}$ & $\epsilon=\frac{8}{255}$ &   $\epsilon=0.3$ \\
Model                          &                  &                          &                          &                  \\
\midrule
CNN                            &            0.991 &          \bfseries 0.985 &          \bfseries 0.973 &            0.000 \\
AdvCNN                         &            0.987 &                    0.978 &                    0.967 &            0.656 \\
CondVAE-NoDrop-Z32             &  \bfseries 0.992 &                    0.984 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-NoDrop-Z32      &            0.988 &                    0.977 &                    0.967 &            0.700 \\
CondVAE-NoDrop-Z128            &  \bfseries 0.992 &                    0.984 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-NoDrop-Z128     &            0.987 &                    0.978 &                    0.967 &            0.697 \\
CondVAE-DropRate02-Z32         &  \bfseries 0.992 &          \bfseries 0.985 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-DropRate02-Z32  &            0.987 &                    0.977 &                    0.967 &            0.702 \\
CondVAE-DropRate02-Z128        &  \bfseries 0.992 &          \bfseries 0.985 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-DropRate02-Z128 &            0.987 &                    0.978 &                    0.968 &            0.697 \\
CondVAE-DropRate05-Z32         &  \bfseries 0.992 &          \bfseries 0.985 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-DropRate05-Z32  &            0.987 &                    0.977 &                    0.967 &            0.699 \\
CondVAE-DropRate05-Z128        &  \bfseries 0.992 &          \bfseries 0.985 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-DropRate05-Z128 &            0.987 &                    0.977 &                    0.967 &            0.695 \\
CondVAE-DropRate08-Z32         &  \bfseries 0.992 &          \bfseries 0.985 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-DropRate08-Z32  &            0.987 &                    0.977 &                    0.967 &  \bfseries 0.703 \\
CondVAE-DropRate08-Z128        &  \bfseries 0.992 &                    0.984 &          \bfseries 0.973 &            0.000 \\
CondVAE-AdvQYX-DropRate08-Z128 &            0.987 &                    0.978 &                    0.967 &            0.695 \\
\bottomrule
\end{tabular}


==> tables/SVHN_BEST_BNN_IN_metrics.tex <==
\begin{tabular}{lcccccc}
\toprule
 &  & Accuracy & ECE & MCE & Brier & Train NLL & Test NLL \\
Dataset & Model &  &  &  &  &  &  \\
\midrule
\multirow[t]{3}{*}{CIFAR10} & TST & 92.586$\pm$0.0208 & 2.18$\pm$0.353 & 14.89$\pm$2.249 & 0.0112$\pm$6e-05 & 0.0573$\pm$0.00023 & 0.2482$\pm$0.004 \\
 & V-TST & 91.095$\pm$0.0604 & 1.52$\pm$0.144 & 14.77$\pm$1.781 & 0.0142$\pm$8e-05 & 0.1125$\pm$0.00099 & 0.3732$\pm$0.00426 \\
 & WRN & 92.53$\pm$nan & 5.88$\pm$nan & 35.84$\pm$nan & 0.013$\pm$nan & 0.1038$\pm$nan & 0.4944$\pm$nan \\
\cline{1-8}
\multirow[t]{3}{*}{SVHN} & TST & 95.103$\pm$0.0074 & 0.43$\pm$0.016 & 25.04$\pm$9.617 & 0.0075$\pm$1e-05 & 0.0439$\pm$6e-05 & 0.1837$\pm$0.00041 \\
 & V-TST & 94.733$\pm$0.0172 & 0.48$\pm$0.067 & 22.63$\pm$6.889 & 0.0083$\pm$2e-05 & 0.059$\pm$0.00025 & 0.2193$\pm$0.00112 \\
 & WRN & 95.068$\pm$nan & 3.48$\pm$nan & 26.61$\pm$nan & 0.0083$\pm$nan & 0.0605$\pm$nan & 0.2869$\pm$nan \\
\cline{1-8}
\bottomrule
\end{tabular}


==> tables/SVHN_BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
 &  & OOD AUROC & OOD FPR95 \\
Dataset & Model &  &  \\
\midrule
\multirow[t]{3}{*}{CIFAR10} & TST & 0.874$\pm$0.0022 & 0.699$\pm$0.009 \\
 & V-TST & 0.722$\pm$0.0053 & 0.824$\pm$0.0065 \\
 & WRN & 0.891$\pm$nan & 0.653$\pm$nan \\
\cline{1-4}
\multirow[t]{3}{*}{SVHN} & TST & 0.935$\pm$0.001 & 0.415$\pm$0.0059 \\
 & V-TST & 0.859$\pm$0.0044 & 0.549$\pm$0.0056 \\
 & WRN & 0.945$\pm$nan & 0.344$\pm$nan \\
\cline{1-4}
\bottomrule
\end{tabular}


==> tables/SVHN_BEST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
 &  & SHIFT ECE & SHIFT MCE \\
Dataset & Model &  &  \\
\midrule
\multirow[t]{3}{*}{CIFAR10} & TST & 11.62$\pm$0.752 & 25.39$\pm$1.74 \\
 & V-TST & 12.89$\pm$0.297 & 21.01$\pm$0.58 \\
 & WRN & 20.27$\pm$nan & 45.06$\pm$nan \\
\cline{1-4}
\multirow[t]{3}{*}{SVHN} & TST & 30.97$\pm$0.069 & 48.39$\pm$0.091 \\
 & V-TST & 35.67$\pm$0.591 & 52.33$\pm$0.587 \\
 & WRN & 47.06$\pm$nan & 80.65$\pm$nan \\
\cline{1-4}
\bottomrule
\end{tabular}


==> tables/SVHN_WRN_BNN_IN_metrics.tex <==
\begin{tabular}{lccccc}
\toprule
{} &         Accuracy &              ECE &               MCE &            Brier &              NLL \\
Model                                  &                  &                  &                   &                  &                  \\
\midrule
CondVAE-WRN-DropRate00-Z128-seed1      &  \bfseries 0.951 &          3.40666 &          37.08554 &          0.00914 &          0.30409 \\
CondVAE-WRN-DropRate00-Z128-seed1-LAST &  \bfseries 0.951 &          4.75482 &          55.83370 &          0.00958 &          0.66210 \\
CondVAE-WRN-DropRate00-Z2-seed1        &          0.94703 &         19.26837 &          46.46904 &          0.01966 &          0.54872 \\
CondVAE-WRN-DropRate00-Z2-seed1-LAST   &          0.94718 &          3.70518 &          45.00727 &          0.00968 &          0.55301 \\
CondVAE-WRN-DropRate00-Z32-seed1       &  \bfseries 0.951 &          2.74709 &          40.23296 &          0.00902 &          0.29070 \\
CondVAE-WRN-DropRate00-Z32-seed1-LAST  &  \bfseries 0.951 &          4.71373 &          46.20408 &          0.00953 &          0.66767 \\
CondVAE-WRN-DropRate02-Z128-seed1      &  \bfseries 0.951 &          3.35452 &          42.86140 &          0.00914 &          0.30326 \\
CondVAE-WRN-DropRate02-Z128-seed1-LAST &  \bfseries 0.951 &          4.81532 &          53.20128 &          0.00967 &          0.68005 \\
CondVAE-WRN-DropRate02-Z2-seed1        &          0.92379 &         25.12192 &          49.66710 &          0.02462 &          0.62480 \\
CondVAE-WRN-DropRate02-Z2-seed1-LAST   &          0.94710 &          3.55559 &          41.39372 &          0.00969 &          0.56377 \\
CondVAE-WRN-DropRate02-Z32-seed1       &  \bfseries 0.951 &  \bfseries 2.657 &          80.63341 &          0.00902 &          0.28951 \\
CondVAE-WRN-DropRate02-Z32-seed1-LAST  &  \bfseries 0.951 &          4.75123 &          67.11942 &          0.00962 &          0.67672 \\
CondVAE-WRN-DropRate05-Z128-seed1      &  \bfseries 0.951 &          3.50953 &          44.12899 &          0.00918 &          0.30794 \\
CondVAE-WRN-DropRate05-Z128-seed1-LAST &  \bfseries 0.951 &          4.77435 &          47.57556 &          0.00963 &          0.66446 \\
CondVAE-WRN-DropRate05-Z2-seed1        &          0.94614 &         21.06963 &          47.81329 &          0.02036 &          0.59285 \\
CondVAE-WRN-DropRate05-Z2-seed1-LAST   &          0.94626 &          3.68839 &          42.95999 &          0.00993 &          0.61591 \\
CondVAE-WRN-DropRate05-Z32-seed1       &  \bfseries 0.951 &          2.78358 &          41.13126 &          0.00901 &          0.29029 \\
CondVAE-WRN-DropRate05-Z32-seed1-LAST  &  \bfseries 0.951 &          4.70878 &          65.10320 &          0.00956 &          0.67731 \\
CondVAE-WRN-DropRate08-Z128-seed1      &  \bfseries 0.951 &          3.48040 &          34.94951 &          0.00914 &          0.30585 \\
CondVAE-WRN-DropRate08-Z128-seed1-LAST &  \bfseries 0.951 &          4.78387 &          50.75230 &          0.00964 &          0.65964 \\
CondVAE-WRN-DropRate08-Z2-seed1        &          0.94526 &         27.45828 &          56.08164 &          0.02590 &          0.66440 \\
CondVAE-WRN-DropRate08-Z2-seed1-LAST   &          0.94607 &          3.84615 &          51.34854 &          0.00990 &          0.59844 \\
CondVAE-WRN-DropRate08-Z32-seed1       &  \bfseries 0.951 &          2.71257 &          41.02060 &          0.00903 &          0.28862 \\
CondVAE-WRN-DropRate08-Z32-seed1-LAST  &  \bfseries 0.951 &          4.72326 &          53.10773 &          0.00956 &          0.66357 \\
WRN-Base                               &  \bfseries 0.951 &          3.48319 &  \bfseries 26.615 &  \bfseries 0.008 &  \bfseries 0.287 \\
\bottomrule
\end{tabular}


==> tables/SVHN_WRN_BNN_OOD_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &        OOD AUROC &        OOD FPR95 \\
Model                                  &                  &                  \\
\midrule
CondVAE-WRN-DropRate00-Z128-seed1      &          0.72295 &          0.68605 \\
CondVAE-WRN-DropRate00-Z128-seed1-LAST &          0.64386 &          0.67485 \\
CondVAE-WRN-DropRate00-Z2-seed1        &          0.65003 &          0.90875 \\
CondVAE-WRN-DropRate00-Z2-seed1-LAST   &          0.63695 &          0.84262 \\
CondVAE-WRN-DropRate00-Z32-seed1       &          0.70423 &          0.66580 \\
CondVAE-WRN-DropRate00-Z32-seed1-LAST  &          0.63419 &          0.75090 \\
CondVAE-WRN-DropRate02-Z128-seed1      &          0.72025 &          0.68385 \\
CondVAE-WRN-DropRate02-Z128-seed1-LAST &          0.67806 &          0.65565 \\
CondVAE-WRN-DropRate02-Z2-seed1        &          0.66266 &          0.92760 \\
CondVAE-WRN-DropRate02-Z2-seed1-LAST   &          0.64076 &          0.85867 \\
CondVAE-WRN-DropRate02-Z32-seed1       &          0.71124 &          0.66980 \\
CondVAE-WRN-DropRate02-Z32-seed1-LAST  &          0.61113 &          0.75770 \\
CondVAE-WRN-DropRate05-Z128-seed1      &          0.72709 &          0.68300 \\
CondVAE-WRN-DropRate05-Z128-seed1-LAST &          0.63880 &          0.67375 \\
CondVAE-WRN-DropRate05-Z2-seed1        &          0.64825 &          0.84445 \\
CondVAE-WRN-DropRate05-Z2-seed1-LAST   &          0.64758 &          0.82863 \\
CondVAE-WRN-DropRate05-Z32-seed1       &          0.71185 &          0.66600 \\
CondVAE-WRN-DropRate05-Z32-seed1-LAST  &          0.62742 &          0.76035 \\
CondVAE-WRN-DropRate08-Z128-seed1      &          0.72941 &          0.67380 \\
CondVAE-WRN-DropRate08-Z128-seed1-LAST &          0.62469 &          0.67545 \\
CondVAE-WRN-DropRate08-Z2-seed1        &          0.64745 &          0.82815 \\
CondVAE-WRN-DropRate08-Z2-seed1-LAST   &          0.65533 &          0.83090 \\
CondVAE-WRN-DropRate08-Z32-seed1       &          0.70964 &          0.66860 \\
CondVAE-WRN-DropRate08-Z32-seed1-LAST  &          0.62515 &          0.76170 \\
WRN_Base                               &  \bfseries 0.945 &  \bfseries 0.344 \\
\bottomrule
\end{tabular}


==> tables/SVHN_WRN_BNN_SHIFT_metrics.tex <==
\begin{tabular}{lcc}
\toprule
{} &         SHIFT ECE &         SHIFT MCE \\
Model                                  &                   &                   \\
\midrule
CondVAE-WRN-DropRate00-Z128-seed1      &          52.30607 &          67.32590 \\
CondVAE-WRN-DropRate00-Z128-seed1-LAST &          57.58225 &          67.01771 \\
CondVAE-WRN-DropRate00-Z2-seed1        &          25.65616 &          41.27033 \\
CondVAE-WRN-DropRate00-Z2-seed1-LAST   &          53.44959 &          69.65095 \\
CondVAE-WRN-DropRate00-Z32-seed1       &          50.56596 &          66.05493 \\
CondVAE-WRN-DropRate00-Z32-seed1-LAST  &          57.03098 &          67.41914 \\
CondVAE-WRN-DropRate02-Z128-seed1      &          52.02913 &          66.67369 \\
CondVAE-WRN-DropRate02-Z128-seed1-LAST &          57.41227 &          67.17263 \\
CondVAE-WRN-DropRate02-Z2-seed1        &          18.31521 &          35.00782 \\
CondVAE-WRN-DropRate02-Z2-seed1-LAST   &          53.13988 &          69.62010 \\
CondVAE-WRN-DropRate02-Z32-seed1       &          50.23307 &          65.56423 \\
CondVAE-WRN-DropRate02-Z32-seed1-LAST  &          56.96033 &          66.50145 \\
CondVAE-WRN-DropRate05-Z128-seed1      &          52.29301 &          66.63759 \\
CondVAE-WRN-DropRate05-Z128-seed1-LAST &          57.54727 &          71.38293 \\
CondVAE-WRN-DropRate05-Z2-seed1        &          23.74106 &          42.30759 \\
CondVAE-WRN-DropRate05-Z2-seed1-LAST   &          53.50530 &          71.01389 \\
CondVAE-WRN-DropRate05-Z32-seed1       &          50.45493 &          65.39259 \\
CondVAE-WRN-DropRate05-Z32-seed1-LAST  &          57.04212 &          67.13098 \\
CondVAE-WRN-DropRate08-Z128-seed1      &          52.32306 &          66.95059 \\
CondVAE-WRN-DropRate08-Z128-seed1-LAST &          57.53531 &          68.51090 \\
CondVAE-WRN-DropRate08-Z2-seed1        &  \bfseries 16.858 &  \bfseries 33.345 \\
CondVAE-WRN-DropRate08-Z2-seed1-LAST   &          53.70234 &          71.85606 \\
CondVAE-WRN-DropRate08-Z32-seed1       &          50.42275 &          65.51433 \\
CondVAE-WRN-DropRate08-Z32-seed1-LAST  &          57.00677 &          67.30442 \\
WRN_Base                               &          47.06308 &          80.65484 \\
\bottomrule
\end{tabular}


==> tables/ViT_ABLATION_BEST_BNN_OOD_metrics.tex <==
\begin{tabular}{llll}
\toprule
 & OOD AUROC & OOD FPR95 \\
Model &  &  \\
\midrule
V-TST, m=10 & 0.832$\pm$0.001 & 0.727$\pm$0.003 \\
V-TST, m=1 & 0.81$\pm$0.001 & 0.769$\pm$0.002 \\
TST & 0.823$\pm$0.002 & 0.751$\pm$0.007 \\
ViT & 0.797 & 0.823 \\
\bottomrule
\end{tabular}


==> tables/ViT_ABLATION_BEST_BNN_SHIFT_metrics.tex <==
\begin{tabular}{llll}
\toprule
 & SHIFT ECE & SHIFT MCE \\
Model &  &  \\
\midrule
V-TST, m=10 & 5.44$\pm$0.35 & 10.05$\pm$0.57 \\
V-TST, m=1 & 10.72$\pm$0.44 & 18.28$\pm$0.75 \\
TST & 8.16$\pm$0.48 & 14.14$\pm$0.82 \\
ViT & 25.46& 45.2\\
\bottomrule
\end{tabular}

